Multiple-Relay Slotted ALOHA: Performance Analysis and Bounds

Wireless random access protocols are attracting a revived research interest as a simple yet effective solution for machine-type communications. In the quest to improve reliability and spectral efficiency of such schemes, the use of multiple receivers has recently emerged as a promising option. We study the potential of this approach considering a population of users that transmit data packets following a simple slotted ALOHA policy to a set of non-cooperative receivers or relays (uplink phase). These, in turn, independently forward - part of - what decoded towards a collecting sink (downlink phase). For an on-off fading channel model, we provide exact expressions for uplink throughput and packet loss rate for an arbitrary number of relays, characterising the benefits of multi-receiver schemes. Moreover, a lower bound on the minimum amount of downlink resources needed to deliver all information collected on the uplink is provided. The bound is proven to be achievable via random linear coding when no constraints in terms of latency are set. We complement our study discussing a family of simple forwarding policies that require no packet-level coding, and optimising their performance based on the amount of available downlink resources. The behaviour of both random linear coding and simplified policies is also characterised when receivers are equipped with finite buffers, revealing non-trivial tradeoffs.

==> acronyms.tex <==
% A
\DeclareAcronym{AWGN}{short = AWGN ,long = additive white gaussian noise}
\DeclareAcronym{ACRDA}{short = ACRDA ,long = asynchronous contention resolution diversity ALOHA}
% B
% C
\DeclareAcronym{CDF}{short = CDF ,long = cumulative distribution function}
\DeclareAcronym{CoMP}{short = CoMP ,long = coordinated multi-point}
\DeclareAcronym{CRA-CC}{short = CRA-CC ,long = CRA-convolutional code}
\DeclareAcronym{CRA-SH}{short = CRA-SH ,long = CRA-shannon bound}
\DeclareAcronym{CRA}{short = CRA ,long = contention resolution ALOHA}
\DeclareAcronym{CRDSA}{short = CRDSA ,long = contention resolution diversity slotted ALOHA}
\DeclareAcronym{CRDSA++}{short = CRDSA++ ,long = contention resolution diversity slotted ALOHA++}
\DeclareAcronym{CSA}{short = CSA ,long = coded slotted ALOHA}
% D
\DeclareAcronym{DAMA}{short = DAMA ,long = demand assigned multiple access}
\DeclareAcronym{DSA}{short = DSA ,long = diversity slotted ALOHA}
% E
\DeclareAcronym{ECRA}{short = ECRA ,long = enhanced contention resolution ALOHA}
\DeclareAcronym{ECRA-SC}{short = ECRA-SC ,long = ECRA selection combining}
\DeclareAcronym{ECRA-MRC}{short = ECRA-MRC ,long = ECRA maximal-ratio combining}
\DeclareAcronym{EGD}{short = EGD ,long = equal-gain diversity}
\DeclareAcronym{ETP}{short = ETP ,long = equal transmission power}
% F
\DeclareAcronym{FEC}{short = FEC ,long = forward error correction}
% G
\DeclareAcronym{GEO}{short = GEO ,long = geostationary orbit}
\DeclareAcronym{GW}{short = GW ,long = gateway}
% H
% I
\DeclareAcronym{IC}{short = IC ,long = interference cancellation}
\DeclareAcronym{IoT}{short = IoT ,long = internet of things}
\DeclareAcronym{IRCRA}{short = IRCRA ,long = irregular repetition contention resolution ALOHA}
\DeclareAcronym{IRSA}{short = IRSA ,long = irregular repetition slotted ALOHA}
% K
% L
% M
\DeclareAcronym{M2M}{short = M2M ,long = machine-to-machine}
\DeclareAcronym{MAC}{short = MAC ,long = medium access}
\DeclareAcronym{MF-TDMA}{short = MF-TDMA ,long = multi-frequency time division multiple access}
\DeclareAcronym{MIMO}{short = MIMO ,long = multiple-input multiple-output}
\DeclareAcronym{MPR}{short = MPR ,long = multi-packet reception}
\DeclareAcronym{MRC}{short = MRC ,long = maximal-ratio combining}
\DeclareAcronym{MTC}{short = MTC ,long = machine-type communications}
% N
% O
\DeclareAcronym{OOF}{short = OOF ,long = on-off fading}
% P
\DeclareAcronym{PDF}{short = PDF ,long = probability density function}
\DeclareAcronym{PER}{short = PER ,long = packet error rate}
\DeclareAcronym{PLR}{short = PLR ,long = packet loss rate}
\DeclareAcronym{PMF}{short = PMF ,long = probability mass function}
\DeclareAcronym{PPC}{short = PPC ,long = perfect power control}
% Q
% R
\DeclareAcronym{RA}{short = RA ,long = Random access}
\DeclareAcronym{RCB}{short = RCB ,long = random coding bound}
\DeclareAcronym{RLC}{short = RLC ,long = random linear coding}
\DeclareAcronym{RTT}{short = RTT ,long = round trip time}
% S
\DeclareAcronym{SA}{short = SA , long = slotted ALOHA}
\DeclareAcronym{SB}{short = SB ,long = Shannon bound}
\DeclareAcronym{SC}{short = SC ,long = selection combining}
\DeclareAcronym{SFP}{short = SFP ,long = simplified forwarding policy}
\DeclareAcronym{SIC}{short = SIC ,long = successive interference cancellation}
\DeclareAcronym{SIR}{short = SIR ,long = signal to interference ratio}
\DeclareAcronym{SNIR}{short = SNIR ,long = signal-to-noise and interference ratio}
\DeclareAcronym{SINR}{short = SINR ,long = signal-to-interference and noise ratio}
\DeclareAcronym{SNR}{short = SNR ,long = signal-to-noise ratio}
% T
\DeclareAcronym{TDMA}{short = TDMA ,long = time division multiple access}
% U
\DeclareAcronym{UCP}{short = UCP ,long = unresolvable collision pattern}
% V
% W
% X
% Y
% Z


==> displaynotation.tex <==
\onecolumn
\section*{Notation}

\bigskip

\begin{center}
\begin{tabular}{ l l l}
\hline \hline
\textbf{Generic} & & \\
$\pr$ & \verb;\pr; & Probability\\
$\load$ & \verb;\load; & Load \\
$\tp$ & \verb;\tp; & Throughput \\
$\tpSA$ & \verb;\tpSA; & Throughput Slotted Aloha\\
$\tpUL$ & \verb;\tpUL; & Throughput Uplink\\
$\tpMax$ & \verb;\tpMax; & Maximum throughput \\
$\tpULMax$ & \verb;\tpULMax; & Maximum Throughput Uplink\\
$\tpDL$ & \verb;\tpDL; & Throughput Downlink\\
$\plrUL$ & \verb;\plrUL; & packet Loss Rate Uplink\\
$\peras$ & \verb;\peras; &  uplink packet erasure probability\\
$\slotTime$ & \verb;\slotTime; &  Slot duration\\
$\slot$ & \verb;\slot; &  Generic slot index\\
\textbf{User} & & \\
$\usersRV$ & \verb;\usersRV; & r.v. describing number of nodes accessing uplink slot\\
$\users$ & \verb;\users; &  number of nodes accessing uplink slot\\
$\usInd$ & \verb;\usInd; &  Generic user index\\
\textbf{Relays} & & \\
$\rxSet$ & \verb;\rxSet; & Set of relays\\
$\nrx$ & \verb;\nrx; & number of relays\\
$\rx$ & \verb;\rx; & considered relay\\
$\setArx$ & \verb;\setArx; & set of decoded packets at relay $\rx$\\
$\rxSubSet$ & \verb;\rxSubSet; & Subset of relays of $\rxSet$\\
$\nrxSubSet$ & \verb;\nrxSubSet; & Cardinality of the set $\rxSubSet$\\
$\subsetrx$ & \verb;\subsetrx; & Generic index of the subset of relays $\subsetrx$\\
$\setAsubset$ & \verb;\setAsubset; & set of decoded packets at relay $\subsetrx$\\
\textbf{Uplink} & & \\
$\ulVal$ & \verb;\ulVal; & Pedix for uplink variables\\
$\ulslot$ & \verb;\ulslot; &  duration of uplink slot\\
$\collRV$ & \verb;\collRV; & r.v. describing number of collected packets\\
$\collrv$ & \verb;\collrv; & number of collected packets\\
$\interfRV$ & \verb;\collRV; & r.v. describing number of interfering packets\\
$\interfrv$ & \verb;\collrv; & number of interfering packets\\
$\numulslot$ & \verb;\numulslot; &  number of observed uplink slots\\
$\psamecoll$ & \verb;\psamecoll; &  probability\\
\textbf{Downlink} & & \\
$\dlVal$ & \verb;\dlVal; & Pedix for downlink variables\\
$\dlslot$ & \verb;\dlslot; &  duration of downlink slot\\
$\numdlslot$ & \verb;\numdlslot; &  number of employed downlink slots (for NC transmissions)\\
$\dlrate$ & \verb;\dlrate; & Downlink Rate\\
$\dlratemin$ & \verb;\dlratemin; & Minimum Downlink Rate\\
$\dlratek$ & \verb;\dlratek; & Downlink Rate to relay $k$\\
$\dltxk$ & \verb;\dltxk; & Fraction of Downlink Rate to relay $k$\\
$\plos$ & \verb;\plos; & packet Loss Rate Downlink\\
$\payload$ & \verb;\payload; & Number of info-bits in considered packets\\
$\erasure$ & \verb;\erasure; & Erasure symbol\\
$\fieldOrd$ & \verb;\fieldOrd; & Field order\\
$\linll$ & \verb;\linll; &  number of linear combination generated a generic relay\\
$\linllK{k}$ & \verb;\linllK{k}; &  number of linear combination generated by the $k$-th relay\\
$\linComb$ & \verb;\linComb; &  vector of linear combinations of packets generated\\
$\linCombK{k}$ & \verb;\linCombK{k}; &  vector of linear combinations of packets generated at relay $k$\\
$\linCombRed$ & \verb;\linCombRed; &  vector of linear combinations of packets generated without erasures\\
$\linCombRedK{k}$ & \verb;\linCombRedK{k}; &  vector of linear combinations of packets generated at relay $k$ without erasures\\
\hline \hline
\end{tabular}
\end{center}

\begin{center}
\begin{tabular}{ l l l}
\hline \hline
\textbf{Downlink} & & \\
$\MxComb$ & \verb;\MxComb; &  Matrix with coefficients for the linear combination of packets sent \\
& & from the relay to the gateway\\
$\MxCombK{k}$ & \verb;\MxCombK{k}; &  Matrix with coefficients for the linear combination of packets sent \\
& & from the relay to the gateway subscript k\\
$\MxCombRed$ & \verb;\MxCombRed; &  Matrix with coefficients for the linear combination of packets sent, \\
& & excluded the all zero columns from the relay to the gateway\\
$\MxCombRedK{k}$ & \verb;\MxCombRedK{k}; &  Matrix with coefficients for the linear combination of packets sent, \\
& & excluded the all zero columns from the relay to the gateway subscript k\\
$\coll$ & \verb;\coll; &  number of collected packets\\
$\collMax$ & \verb;\collMax; &  Maximum number of collected packets\\
$\collK{k}$ & \verb;\collK{k}; &  number of collected packets at relay $k$\\
$\colVec$ & \verb;\colVec; &  vector of collected packets\\
$\colVecK{k}$ & \verb;\colVecK{k}; &  vector of collected packets at relay $k$\\
$\colVecNum$ & \verb;\colVecNum; &  vector of number of collected packets\\
$\USet$ & \verb;\USet; & Set\\
$\LSet$ & \verb;\LSet; & Set\\
\textbf{Simplified Forwarding Policies} & & \\
$\capDL$ & \verb;\capDL; &  downlink capacity\\
$\dropVec$ & \verb;\dropVec; &  vector of dropping probabilities\\
$\dropij{k}{j}$ & \verb;\dropij{k}{j}; &  $j$-th dropping probability for relay $k$\\
$\arrRate{k}$ & \verb;\arrRate{k}; &  arrival rate at the $k$-th relay\\
$\coeffA$ & \verb;\coeffA; &  coefficient for formulas in forwarding policies\\
$\coeffB$ & \verb;\coeffB; &  coefficient for formulas in forwarding policies\\
$\coeffC$ & \verb;\coeffC; &  coefficient for formulas in forwarding policies\\
$\coeffD$ & \verb;\coeffD; &  coefficient for formulas in forwarding policies\\
$\coeffE$ & \verb;\coeffE; &  coefficient for formulas in forwarding policies\\
\textbf{Downlink Finite Buffer} & & \\
$\rankk$ & \verb;\rankk; & Matrix rank\\
$\rankK{k}$ & \verb;\rankK{k}; & Matrix rank of submatrix $k$\\
$\mxCol$ & \verb;\mxCol; & Matrix col number\\
$\mxColK{k}$ & \verb;\mxColK{k}; & Matrix col number of submatrix $k$\\
$\Id$ & \verb;\Id; & Identity matrix\\
$\MxA$ & \verb;\MxA; & One matrix\\
$\MxB$ & \verb;\MxB; & One matrix\\
$\MxUone$ & \verb;\MxUone; & One matrix\\
$\MxUtwo$ & \verb;\MxUtwo; & One matrix\\
$\MxL$ & \verb;\MxL; & One matrix\\
$\collSinkone$ & \verb;\collSinkone; & Number of decoded packet at the sink, from relay $1$\\
$\collSinktwo$ & \verb;\collSinktwo; & Number of decoded packet at the sink, from relay $2$\\
$\collSinkboth$ & \verb;\collSinkboth; & Number of decoded packet at the sink, from both relays\\
$\collSinkoneRV$ & \verb;\collSinkoneRV; & RV corr. number of decoded packet at the sink, from relay $1$\\
$\collSinktwoRV$ & \verb;\collSinktwoRV; & RV corr. number of decoded packet at the sink, from relay $2$\\
$\collSinkbothRV$ & \verb;\collSinkbothRV; & RV corr. number of decoded packet at the sink, from both relays\\
$\MxM$ & \verb;\MxM; & Generic matrix\\
$\state$ & \verb;\state; & State in the Markov chain\\
$\eo$ & \verb;\eo; & First bases vector in $\mathbb N^3$\\
$\et$ & \verb;\et; & Second bases vector in $\mathbb N^3$\\
$\etr$ & \verb;\etr; & Third bases vector in $\mathbb N^3$\\
$\Tx$ & \verb;\Tx; & Helper Throughput value\\
$\st$ & \verb;\st; & Transition probability in Markov chain\\
\textbf{Appendix} & & \\
$\x$ & \verb;\x; & x as dummy variable\\
$\hSet$ & \verb;\hSet; & Subset of relays\\
$\vSet$ & \verb;\vSet; & Subset of relays\\
\textbf{Others} & & \\
$\sv$ & \verb;\sv; & helper variable in the context of weak low of large number\\
$\dummy$ & \verb;\dummy; & dummy variable for counting in summations\\

\hline \hline
\end{tabular}
\end{center}

\twocolumn









\clearpage 
